Representation Learning by Rotating Your Faces

The large pose discrepancy between two face images is one of the fundamental challenges in automatic face recognition. Conventional approaches to pose-invariant face recognition either perform face frontalization on, or learn a pose-invariant representation from, a non-frontal face image. We argue that it is more desirable to perform both tasks jointly to allow them to leverage each other. To this end, this paper proposes a Disentangled Representation learning-Generative Adversarial Network (DR-GAN) with three distinct novelties. First, the encoder-decoder structure of the generator enables DR-GAN to learn a representation that is both generative and discriminative, which can be used for face image synthesis and pose-invariant face recognition. Second, this representation is explicitly disentangled from other face variations such as pose, through the pose code provided to the decoder and pose estimation in the discriminator. Third, DR-GAN can take one or multiple images as the input, and generate one unified identity representation along with an arbitrary number of synthetic face images. Extensive quantitative and qualitative evaluation on a number of controlled and in-the-wild databases demonstrate the superiority of DR-GAN over the state of the art in both learning representations and rotating large-pose face images.

==> PAMI_2017_DR_GAN_exp_image_synthesis.tex <==

\SubSection{Image Synthesis}
\label{sec:syn}

\begin{figure}[t!]
\begin{center}
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ @{}c@{\hskip 1.5mm}c@{}c@{}c@{}c@{}c@{}c@{\hskip 1.5mm}c@{}}
\toprule
Input && $0^o$ & $15^o$ & $30^o$ & $45^o$ & $60^o$ \\ \midrule

&& 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l231_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l231_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l231_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l231_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l231_10.png} & L2 \\

\includegraphics[width=\acollumsize]{img/MTPIE_visual/i231_input.png} && 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i231_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i231_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i231_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i231_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i231_10.png}& DR-GAN\\
&&
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt231_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt231_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt231_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt231_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt231_10.png}& GT \\ \midrule
& &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l275_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l275_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l275_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l275_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l275_10.png}& L2 \\

\includegraphics[width=\acollumsize]{img/MTPIE_visual/i275_input.png} && 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i275_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i275_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i275_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i275_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i275_10.png}& DR-GAN \\
&&
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt275_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt275_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt275_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt275_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt275_10.png}& GT\\
\iffalse
\midrule 
&&
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l272_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l272_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l272_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l272_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/l272_10.png}& L2\\

\includegraphics[width=\acollumsize]{img/MTPIE_visual/i272_2.png}
&&
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i272_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i272_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i272_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i272_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/i272_10.png}& GAN\\
&&
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt272_6.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt272_7.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt272_8.png} &
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt272_9.png} & 
\includegraphics[width=\acollumsize]{img/MTPIE_visual/gt272_10.png}& GT\\ 
\fi
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{\small Visual comparison of face synthesis on Multi-PIE. For each input image, we compare synthesized images of $L2$ loss (top), adversarial loss (middle), and their ground truth (bottom).} %FIXME: correct input image} %The noise $z$ is set to be a zero vector in all cases.
\label{fig:GANvsL2}\figvspace\vspace{-4mm}
\end{center}
\end{figure}

\Paragraph{Decoder feature}
Visualize feature in Fig.~\ref{fig:decoder_feature}


\begin{figure}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Visuallization of features in different layers, pose code}
\label{fig:decoder_feature}
\end{figure}

\PlaceHolderText{$G_{dec}$ feature}

\Paragraph{Adversarial Loss vs.~$L2$ Loss}
Prior work~\cite{zhu2013deep, yim2015rotating, yang2015weakly} on face rotation normally employ the $L2$ loss to learn a mapping between two views. %from a face image with an arbitrary view to a target view.
%In contrast, by integrating the adversarial loss, we expect to learn a more discriminative representation for better recognition, and a more generative representation for better face synthesis.
To compare the $L2$ loss with our adversarial loss, we train a model where $G$ is supervised by an $L2$ loss on the ground truth face with the target view. %, instead of the adversarial loss in $D$. 
The training process is kept the same for a fair comparison. %of two losses. and parameter settings
%Figure~\ref{fig:GANvsL2} shows the visual comparison of the synthesized faces. % with different views from our generator networks trained with $L2$ loss and adversarial loss. 
As shown in Fig.~\ref{fig:GANvsL2}, DR-GAN can generate far more realistic faces that are similar to the ground truth faces in all views. 
Meanwhile, images synthesized by the $L2$ loss cannot maintain high frequency components and are blurry. 
In fact, $L2$ loss treats each pixel equally, which leads to the loss of discriminative information. 
This inferior synthesis is also reflected in the lower PIFR performance in Tab.~\ref{tab:MTPIE_results}. 

\Paragraph{Interpolation of Variables}
Taking two images of different subjects $\mathbf{x}_1, \mathbf{x}_2$, we extract features $f(\mathbf{x}_1)$ and $f(\mathbf{x}_2)$ from $G_{enc}$. 
The interpolation between $f(\mathbf{x}_1)$ and $f(\mathbf{x}_2)$ can generate many representations, which can be fed to $G_{dec}$ to synthesize face images. 
In Fig.~\ref{fig:interpolation} (a), the top row shows a transition from a male subject with beard and glasses to a female without these adjectives. 
%The second and third rows also show the transition from a person without glasses to the one with glasses. 
Similar to~\cite{radford2015unsupervised}, these smooth semantic changes indicate that the model has learned essential identity representations for image synthesis. %FIXME why cite this paper here?

During training, we use a one-hot vector $\bf{c}$ to specify the {\it discrete} pose of the synthetic image. 
During testing, we could also interpolate between two neighboring pose codes, to generate face images with {\it continuous} poses. %, whose pose code is the weighted average of two neighboring pose codes. 
%In order to do this, we compute a new pose code as the weighted average of two neighboring pose codes. 
As in Fig.~\ref{fig:interpolation} (b), this leads to smooth pose transition from one view to many views {\it unseen} to the training set. %that have not been seen in the training set. 

We also interpolate the noise $\bf{z}$.
We synthesize frontal faces at ${\bf{z}}=-{\bf{1}}$ and ${\bf{z}}={\bf{1}}$ (a vector of all $1$s) and interpolate between two ${\bf{z}}$.
Given the fixed identity representation and pose code, the synthetic images are identity-preserving frontal faces. 
For better visualization, we show the difference of the images w.r.t.~the image generated by ${\bf{z}}=-{\bf{1}}$. 
As in Fig.~\ref{fig:interpolation} (c), $\bf{z}$ models less significant face variations. 


\Paragraph{Face Rotation}
Our generator is trained to be a face rotator.
%Given one or multiple face images with arbitrary poses, we can generate multiple identity-preserving faces at different views. 
Face rotation on Multi-PIE is shown in Fig.~\ref{fig:GANvsL2} and Fig.~\ref{fig:interpolation}.
Figure~\ref{fig:CFP_Visual} shows the face frontalization on CFP. 
Given an input image at large poses even extreme profile, DR-GAN can generate a realistic frontal face that is very similar to the real frontal face.
To the best of our knowledge, this is the first work that is able to {\it frontalizate a profile-view in-the-wild face image}. 
Figure~\ref{fig:IJBA_Visual} shows the face rotation on IJB-A with various number of input images. %, which can be in very low quality. 
During face rotation, the identity is preserved and pose-view is changed exactly to the target pose, indicating that the learnt representation is largely disentangled with other variations and the pose code entirely determines the synthesized pose.
We want to emphasize that it is extremely difficult to {\it fuse multiple in-the-wild face images into a single frontal face image}, when the input images have diverse and large variations in poses, expressions, lightings and resolutions. 
We believe that this is the first time such a fusing capability has been demonstrated on challenging databases such as IJB-A.


%Figure~\ref{fig:MTPIE_visual} shows the face rotation results on Multi-PIE.
%We can generate faces that are similar to the ground truth images. 
%During face rotation, the identity is preserved and pose-view is changed exactly to the target pose, indicating again that the learnt representation is largely disentangled with other variations and the pose code entirely determines the synthesized pose.
%Figure~\ref{fig:CFP_Visual} shows the face rotation results on CFP. 
%DR-GAN can generate realistic images with the same identity as the input even in unconstrained settings. 

\Paragraph{Representation vs.~Synthetic Image}
DR-GAN can simultaneously extract a representation, and generate a frontal face of the same subject - both are useful for PIFR. 
The representation is directly used via the cosine distance metric. 
The synthetic image can be fed to a pretrained face recognition model, with an architecture similar to CASIA-Net~\cite{yi2014learning} to extract identity features for PIFR. 
The performance comparison is reported in Tab.~\ref{tab:CFP_results}. 
It appears that the representation is more effective. 
However, the synthetic images are visually appealing, and can be promising in law enforcement practice, especially given their notable PIFR performance.
%that their PIFR performance is comparable to the state of the art.
%The performance of the synthetic images is close to the state-of-the-art methods, which shows their promise in law enforcement practice. 
%It's also worth to note that using synthesized frontal images has comparable performance as using original images on the same CNN, which has $97.12\%$ and $90.82\%$ for frontal-frontal and frontal-profile respectively. %with a slightly improvement is profile images. 
%This shows the promise of using synthetic images in law enforcement practice. 




%\SubSection{Feature is pose-invariance}
%Plot PCA our feature and feature train by soft-max on MTPIE



%\SubSection{Feature is pose-invariance}
%Plot PCA our feature and feature train by soft-max on MTPIE

\Paragraph{Multi-image combination} 
We also explore the effect of the number of input images on the image synthesis task. From a template of one subject with $20$ images, we sample different subsets of this template with $2, 5, 10, 15$ images respectively. Figure~\ref{fig:IJBA_Visual3} shows synthetic face images of these subsets. As more images are used as the input, DR-GAN can generate images with the more precise identity.

\begin{figure*}[h!]
\begin{center}
\small
\setlength{\tabcolsep}{2pt}
\begin{tabular}{ cccccccccccccccccccc }

2 &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_01.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_02.png}
&&
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_5.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_6.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_7.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_8.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_9.png} && \\
5 &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_03.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_04.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_05.png}
&&
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_125.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_126.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_127.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_128.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_129.png} && \\
10 &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_06.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_07.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_08.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_09.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_10.png}
&&
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_365.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_366.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_367.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_368.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_369.png} && \\

15 &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_11.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_12.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_13.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_14.png}
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_15.png}
&&
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_455.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_456.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_457.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_458.png} &
\includegraphics[width=\IJBAcollumsize]{img/IJBA_DontKnow/img_459.png} && \\

$\#$ images & input images && $-30^\circ$ & $-15^\circ$ & $0^\circ$ & $15^\circ$ & $30^\circ$

\end{tabular}
\vspace{-2mm}
\caption{\small Face rotation on IJB-A with different numbers of input images of the same subject. 
We show the number of input images (left), the input images from the templates (middle), and the synthetic images at $5$ different poses (right). For each row, the inputs are images from the same row and all above.}
%Face rotation on CFP for left profile (left) and right profiles (right) to $4$ different poses and frontal faces of the same person.}
\label{fig:IJBA_Visual3}\figvspace
\end{center}
\end{figure*}

\input{PAMI_2017_DR_GAN_exp_interpolation_fig.tex}
\input{PAMI_2017_DR_GAN_exp_Multi_PIE_fig.tex}
\input{PAMI_2017_DR_GAN_exp_CFP_fig.tex}
\input{PAMI_2017_DR_GAN_exp_IJBA_fig.tex}

==> PAMI_2017_DR_GAN_exp_representatoin_learning.tex <==

\SubSection{Representation Learning}

\Paragraph{Bounding experiment} Using different $D_{id}$ with different quality.  Results are shown in fig..~\ref{fig:bounding}

\PlaceHolderText{Bounding experiment}


\Paragraph{Boosting by switching $G_{enc}$ to $D_{d}$}
Results are shown in tab.~\ref{tab:boosting} 
\PlaceHolderText{Boosting using three $D_d$}

\begin{table}
\begin{center}
\caption{Recognition performance of  $G_{enc}$ when keep switching to $D_{d}$. (Iteration 0, $G_{enc}$ is trained purely with softmax loss) }
\label{tab:boosting}
\small
%\resizebox{0.99\linewidth}{!}{
\begin{tabular}{ lcccccccccc }
\toprule
 Iter                 & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ \midrule
 Recognition rate(\%) &  00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\
\bottomrule
\end{tabular}
\end{center}\figvspace\vspace{-2mm}
\end{table}


\Paragraph{Measure generative and discriminative}
Results are shown in tab.~\ref{tab:gen_dis} 


\begin{table}
\begin{center}
\caption{ Generative measurement comparision }
\label{tab:gen_dis}
%\small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|*{5}{c}}\toprule
\backslashbox{Feature}{Rec}
&\makebox[3em]{$G_{enc}$}&\makebox[3em]{$D_{d}$}&\makebox[3em]{Finetune}&\\
\midrule
$G_{enc}$ & 84.6 & 83.2 & 00.0 \\
$D_{d}$ & 79.3 & 78.1 & 00.0 \\
\bottomrule
\end{tabular}
}
\end{center}\figvspace
\end{table}



\Paragraph{Single vs.~Multiple Training Images}
\label{sec:single_vs_multiple_training}
We evaluate the effect of the number of training images ($n$) per subject on the face recognition performance. 
Specifically, with the same training set, we train three models with $n=1,4,6$, where $n=1$ denotes single-image DR-GAN and $n>1$ denotes multi-image DR-GAN.
%The learnt representation in each model are used for face recognition and 
The testing performance on CFP using $f({\bf{x}})$ of each model are shown in Tab.~\ref{tab:CFP_results_1}.
We observe the advantage of multi-image DR-GAN over the single-image counterpart, which attributes to more constraints in learning $G_{enc}$ that leads to a better representation. 
%We compare single-image DR-GAN with multi-image DR-GAN by using the learnt representation for face recognition. 
%We train three models using different numbers of input images per subject: $n=1,4,6$, with $n=1$ denoting the single-image DR-GAN, 
%Table.~\ref{tab:CFP_results} compares the performance on CFP. 
%It demonstrates the advantage of training with multi-image DR-GAN over the single-image counterpart.
%Training with multiple images per subject applies more constraints in learning $G_{enc}$, which leads to a better representation. 
%not only enhances the model's ability to handle multiple test images, but also 
However, we do not keep increasing $n$ due to the limited computation capacity. 
In the rest of the paper, we use multi-image DR-GAN with $n=6$ unless specified. 

%the other models are multi-image DR-GAN.
%We also note that as $n$ increases, the performance improves due to more constraints in learning.
%As mentioned in Sec.~\ref{sec:multiple_img_model}, during training, the number of input images per subject is keep fixed as $n$, and drop-out is applied to confidence coefficient to replicate variance in the input number. 
%Based on the same training set, we train three models using different numbers of input images per subject, $n$, to explore its affect on the performance. 
%The advance of multiple input models over single input counterpart shows that training with multiple input help to sharp our model to learn better representation. Using more input images during training stage also help to improve the performance.

%\begin{table}[t!]
%\caption{\small Face verification accuracy ($\%$) on CFP with different numbers of training images per subject ($n$). }
%%We stop at $n=6$ due to computation capacity.}
%\label{tab:multi_input_training}\figvspace
% \begin{center}
% \small
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{ ccccc }
%\toprule
%$n$ & Frontal-Frontal & Frontal-Profile \\ \midrule
%1 & $97.13\pm0.68$ & $90.82\pm0.28$ \\ 
%%2 & xx.xx $\pm$ x.xx & xx.xx$\pm$x.xx \\ 
%4 & $97.86\pm0.75$ & $92.93\pm1.39$ \\ 
%6 & $\mathbf{97.84}\pm0.79$ & ${\mathbf{93.41}}\pm1.17$ \\ 
%\bottomrule
%\end{tabular}
%%}
%\end{center}\figvspace
%\end{table}

\begin{table}[t!]
\footnotesize
\caption{\small{Performance comparison on CFP.}} 
\label{tab:CFP_results_1}
\vspace{-3mm}
\begin{center}
\begin{tabular}{ lcc}
\toprule 
Method & Frontal-Frontal & Frontal-Profile\\ \midrule
%Sengupta \etal~\cite{sengupta2016frontal} & $96.40\pm0.69$ & $84.91\pm1.82$ \\
%Sankarana \etal~\cite{sankaranarayanan2016triplet} & $96.93\pm0.61$ & %$89.17\pm2.35$ \\ 
%Chen \etal~\cite{chen2016fisher} & ${\bf{98.67}}\pm0.36$ & $91.97\pm1.70$ \\
%Human & $96.24\pm0.67$ & $94.57\pm1.10$ \\ \midrule
%DR-GAN: synthetic & $97.08\pm0.62$ & $91.02\pm1.59$ \\
DR-GAN: n=$1$ & $97.13\pm0.68$ & $90.82\pm0.28$ \\ 
DR-GAN: n=$4$ & $97.86\pm0.75$ & $92.93\pm1.39$ \\ 
DR-GAN: n=$6$ & $97.84\pm0.79$ & ${\bf{93.41}}\pm1.17$ \\ 
\bottomrule
\end{tabular}
\end{center}
\figvspace
\end{table}

\Paragraph{Single vs.~Multiple Testing Images}
\label{sec:single_vs_multiple_test}
We also evaluate the effect of the number of testing images ($n_t$) per subject on the face recognition performance on Multi-PIE. 
We mimic IJB-A to generate image sets as the probe set while the gallery set remains the same with one image per subject. 
Specifically, from the Multi-PIE probe set, we select a subsect $\mathbb{P}_0$ of images with large poses ($30^{\circ}$ to $60^{\circ}$), which are used to form $5$ different probe sets $\{\mathbb{P}_i\}_{i=1}^5$ with $n_t$ ranging from $1$ to $5$.
First, we randomly select one image per subject from $\mathbb{P}_0$ to form $\mathbb{P}_1$. 
%We now compare performance of DR-GAN on Multi-PIE when testing on multiple images per subject.
%We mimic IJB-A to generate image sets as the probes for face recognition. 
%Specifically, we first select a subset $\mathbb{P}_0$ of images with large poses (absolute pose in the range $30^o$ to $60^o$) from our probe set. 
%We then form five different probe sets from $\mathbb{P}_0$ where the number of images per probe range from $1$ to $5$. 
%First, we have $\mathbb{P}_1 = \mathbb{P}_0$. 
Second, based on $\mathbb{P}_1$, we construct $\mathbb{P}_2$ by adding one random image of each subject from $\mathbb{P}_0$. % with the same identity to each probe image, resulting in two images per subject. 
We construct $\mathbb{P}_{3}$, $\mathbb{P}_{4}$, $\mathbb{P}_{5}$ in a similar way. 
%The gallery is the same for all five sets. 

We compare three combinations of models and decision metrics: (i) single-image DR-GAN with the averaged cosine distances of $n_t$ representations, (ii) multi-image DR-GAN with the averaged cosine distances of $n_t$ representations, and (iii) multi-image DR-GAN with the cosine distance of the fused representation. 
As shown in Tab.~\ref{tab:multi_input_testing}, comparing (ii) and (iii), using the coefficients learned by the network for representation fusion is superior over the conventional score averaging. 
There is a consistent improvement of $\sim$$0.5\%$.
While there is some improvement from (i) to (ii), the margin decreases as $n_t$ increases.

\begin{table}[t!]
\footnotesize
\caption{\small Identification rates of three approaches on Multi-PIE.}
\label{tab:multi_input_testing} \vspace{-3mm}
\begin{center}
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{ lccccc }
\toprule
$n_t$ & $1$ & $2$ & $3$ & $4$ & $5$ \\ \midrule
single-image (avg.) & $84.6$ & $91.8$ & $94.1$ & $95.3$ & $95.8$ \\ 
multi-image (avg.) & $85.9$ & $92.4$ & $94.5$ & $95.5$ & $95.9$ \\ 
multi-image (fuse) & $85.9$ & $92.8$ & $95.1$ & $96.0$ & $96.5$ \\ 
\bottomrule
\end{tabular}
}
\end{center}\figvspace
\end{table}




\Paragraph{Confidence coefficient analysis} 
Results are shown in fig.~\ref{fig:confidence_coefficient}
\PlaceHolderText{Confidence coefficient analysis} 


\begin{figure*}[t!]
\begin{center}
\includegraphics[trim=0 0 100 105, clip, width=0.98\linewidth]{img/coefficient/coefficient_distribution.pdf}
\end{center}
   \caption{Confidence coefficient analysis figure.}
\label{fig:confidence_coefficient}
\end{figure*}

\begin{figure}[t!]
\begin{center}
\includegraphics[trim=140 225 155 225, clip, width=0.8\linewidth]{img/coefficient/corelation.pdf}
\end{center}
   \caption{Confidence coefficient analysis figure. Correlation $0.69$.}
\label{fig:confidence_coefficient_correlation}
\end{figure}

\Paragraph{Results on Benchmark Databases}
We compare our method with state-of-the-art face recognition methods on Multi-PIE, CFP, and IJB-A. 
Table~\ref{tab:MTPIE_results} shows the face identification performance on Multi-PIE compared to the methods with the same setting. 
Our method shows a significant improvement for large-pose faces. 
The variation of recognition rates across different poses is much smaller than the baselines, which suggests that our learnt representation is more robust to pose variation. 
%This shows our learnt representation is more robust to pose variations. 
% than previous methods.

\begin{table*}[t!]
\caption{\small Identification rate ($\%$) comparison on Multi-PIE.}
\label{tab:MTPIE_results} \vspace{-4mm}
\begin{center}
\small
%\resizebox{0.7\linewidth}{!}{
\begin{tabular}{ lccccccccccc }
\toprule
& $-60^o$ & $-45^o$ & $-30^o$ & $-15^o$ & $0^o$ & $15^o$ & $30^o$ & $45^o$ & $60^o$ & \hspace{1mm} & Average\\ \midrule
Zhu \etal~\cite{zhu2013deep} & 49.3 & 66.1 & 78.9 & 91.4 & 94.3 & 90.0 & 82.5 & 62.0 & 42.5 & & 72.9 \\
Zhu \etal~\cite{zhu2014multi} & 60.2 & 75.2 & 83.4 & 93.3 & 95.7 & 92.2 & 83.9 & 70.6 & 60.0 & & 79.3 \\
Yim \etal~\cite{yim2015rotating} & 63.2 & 80.4 & 88.1 & $\mathbf{94.5}$ & $\mathbf{99.5}$ & $\mathbf{95.4}$ & 88.9 & 79.4 & 60.6 & & 83.3 \\ 
Using $L2$ loss & 59.8 & 73.1 & 81.3 & 91.4 & 95.1 & 90.2 & 84.0 & 72.3 & 55.9 & & 78.3 \\
\midrule
DR-GAN & $\mathbf{83.8}$ & $\mathbf{86.6}$ & $\mathbf{89.9}$ & 93.5 & 97.0 & 94.5 & $\mathbf{90.3}$ & $\mathbf{85.8}$ & $\mathbf{82.5}$ && $\mathbf{89.2}$ \\
\bottomrule
\end{tabular}%}
\end{center}\figvspace
\end{table*}

%\begin{table}[t!]
%\caption{\small Benchmark comparison on Multi-PIE. }
%%The $L2$ loss will be covered in Sec.~\ref{sec:syn}.}
%\label{tab:MTPIE_results} \vspace{-3mm}
%\begin{center}
%\small
%\resizebox{0.99\linewidth}{!}{
%\begin{tabular}{ lcccccccccc }
%\toprule
%Method & $0^{\circ}$ & $15^{\circ}$ & $30^{\circ}$ & $45^{\circ}$ & $60^{\circ}$ &  Average\\ \midrule
%Zhu \etal~\cite{zhu2013deep} & $94.3$ & $90.7$ & $80.7$ & $64.1$ & $45.9$  & $72.9$ \\
%Zhu \etal~\cite{zhu2014multi} & $95.7$ & $92.8$ & $83.7$ & $72.9$ & $60.1$  & $79.3$ \\
%Yim \etal~\cite{yim2015rotating} & $\mathbf{99.5}$ & $\mathbf{95.0}$ & $88.5$ & $79.9$ & $61.9$ & $83.3$ \\ 
%Using $L2$ loss & $95.1$ & $90.8$ & $82.7$ & $72.7$ & $57.9$  & $78.3$ \\
%\midrule
%DR-GAN & $97.0$ & $94.0$ & $\mathbf{90.1}$ & $\mathbf{86.2}$ & $\mathbf{83.2}$ & $\mathbf{89.2}$ \\
%\bottomrule
%\end{tabular}}
%\end{center}\figvspace\vspace{-2mm}
%\end{table}

We also evaluate our method on more challenging databases including CFP and IJB-A. 
Table~\ref{tab:CFP_results} shows the comparison on CFP evaluated with Accuracy, Equal Error Rate(EER), and Area Under the Curve (AUC). 
Results are reported with the average face verification accuracy with standard deviation over $10$ folds. 
%Verification results on CFP, including the average Accuracy, Equal Error Rate(EER) and Area Under the Curve (AUC), are reported in Tab.~\ref{tab:CFP_results}. 
We achieve comparable performance on frontal-frontal verification while having $\sim$$1.4\%$ improvement on the frontal-profile verification. 

Table~\ref{tab:ijb-a} shows the performance of both face identification and verification on IJB-A. 
DR-GAN achieves comparable performance to state-of-the-art methods. 
Further, the proposed fusion scheme via learnt coefficients is superior to the averaged cosine distances of representations.
These in-the-wild results show the power of DR-GAN for PIFR. 
%This again shows the power of DR-GAN in PIFR.

\begin{table*}[t!]
\footnotesize
\caption{Performance comparison on CFP dataset.} 
\label{tab:CFP_results}\vspace{-3mm}
\begin{center}
\begin{tabular}{ lcccccc}
\toprule 
& \multicolumn{3}{c}{Frontal-Frontal} & \multicolumn{3}{c}{Frontal-Profile} \\ \midrule 
Method & Accuracy($\%$) & EER($\%$) & AUC($\%$) & Accuracy($\%$) & EER($\%$) & AUC($\%$) \\ \midrule
Sengupta \etal~\cite{sengupta2016frontal} & $96.40\pm0.69$ & $3.48\pm0.67$ & $99.43\pm0.31$ & $84.91\pm1.82$ & $14.97\pm1.98$ & $93.00\pm1.55$ \\
Sankarana \etal~\cite{sankaranarayanan2016triplet} & $96.93\pm0.61$& $2.51\pm0.81$ & $99.68\pm0.16$ & $89.17\pm2.35$ & $8.85\pm0.99$ & $97.00\pm0.53$ \\ 
Chen \etal~\cite{chen2016fisher} & ${\bf{98.67}}\pm0.36$ & ${\bf{1.40}}\pm0.37$ & ${\bf{99.90}}\pm0.09$ & $91.97\pm1.70$ & $8.00\pm1.68$ & $97.70\pm0.82$ \\
Human & $96.24\pm0.67$ & $5.34\pm1.79$ & $98.19\pm1.13$ & $94.57\pm1.10$ & $5.02\pm1.07$ & $98.92\pm0.46$\\ \midrule
DR-GAN & $97.84\pm0.79$ & $2.22\pm0.09$ & $99.72\pm0.02$ & ${\bf{93.41}}\pm1.17$ & ${\bf{6.45}}\pm0.16$ & ${\bf{97.96}}\pm0.06$ \\

DR-GAN (color + split) & $97.96\pm0.75$ & $0.00\pm 0.00$ & $00.00\pm 0.00$ & ${\bf{93.39}}\pm1.23$ & ${\bf{0.00}}\pm0.00$ & ${\bf{00.00}}\pm0.00$ \\

DR-GAN (color + split+interpolation) & $98.13\pm0.81$ & $0.00\pm 0.00$ & $00.00\pm 0.00$ & ${\bf{93.64}}\pm1.51$ & ${\bf{0.00}}\pm0.00$ & ${\bf{00.00}}\pm0.00$ \\

 
\bottomrule
\end{tabular}
\end{center}
\figvspace
\end{table*}

\begin{table}[t!]
\caption{\small{Performance comparison on IJB-A.}}
\vspace{-3mm}
\footnotesize
\begin{center}
\begin{tabular}{@{\hskip .5mm}l@{\hskip 1.5mm}c@{\hskip 1.5mm}c@{\hskip 1.5mm}c@{\hskip 1.5mm}c@{\hskip .5mm}}
\toprule
& \multicolumn{2}{c}{Verification} & \multicolumn{2}{c}{Identification} \\ \cmidrule(r){2-3} \cmidrule(r){4-5}
Method & @FAR=$.01$ & @FAR=$.001$ & @Rank-$1$ & @Rank-$5$ \\ \midrule
OpenBR~\cite{klare2015pushing} & $23.6\pm0.9$ & $10.4\pm1.4$ & $24.6\pm1.1$ & $37.5\pm0.8$ \\
GOTS~\cite{klare2015pushing} & $40.6\pm1.4$ & $19.8\pm0.8$ & $44.3\pm2.1$ & $59.5\pm2.0$ \\
Wang \etal~\cite{wang2016face} & $72.9\pm3.5$ & $51.0\pm6.1$ & $82.2\pm2.3$ & $93.1\pm1.4$ \\ 
%DCNNs~\cite{chen2016unconstrained}& \textcolor{blue}{$83.8\pm4.2$} & \textendash & \textcolor{blue}{$90.3\pm1.2$} & \textcolor{blue}{$96.5\pm0.8$} \\
PAM~\cite{masi2016pose} & $73.3\pm1.8$ & ${\bf{55.2}}\pm3.2$ & $77.1\pm1.6$ & $88.7\pm0.9$ \\
DCNN~\cite{chen2016unconstrained} & ${\bf{78.7}}\pm4.3$ & \textendash & $85.2\pm1.8$ & $93.7\pm1.0$ \\ \midrule
%PAMs~\cite{masi2016pose} & $82.6\pm1.8$ & $65.2\pm3.7$ & $84.0\pm1.2$ & $92.5\pm0.8$ \\ \midrule
DR-GAN (avg.) & $75.5\pm2.8$ & $51.8\pm6.8$ & $84.3\pm1.3$ & $93.2\pm0.8$ \\
DR-GAN (fuse) & $77.4\pm2.7$ & $53.9\pm4.3$ & ${\bf{85.5}}\pm1.5$ & ${\bf{94.7}}\pm1.1$ \\ \bottomrule
\end{tabular}
\end{center}
\eqnvspace
%The best performance for one/multiple models is highlighted in \textcolor{red}{red}/\textcolor{blue}{blue} respectively. } 
\label{tab:ijb-a}
\vspace{-2mm}
\end{table}
